A Tighter Convergence Proof of Reverse Experience Replay

In reinforcement learning, Reverse Experience Replay (RER) is a recently proposed algorithm that attains better sample complexity than the classic experience replay method. RER requires the learning algorithm to update the parameters through consecutive state-action-reward tuples in reverse order. However, the most recent theoretical analysis only holds for a minimal learning rate and short consecutive steps, which converge slower than those large learning rate algorithms without RER. In view of this theoretical and empirical gap, we provide a tighter analysis that mitigates the limitation on the learning rate and the length of consecutive steps. Furthermore, we show theoretically that RER converges with a larger learning rate and a longer sequence.

==> tex/12.main_thorem_proof.tex <==
\section{Proof in Theorem~\ref{th:main}}

By linearity of expectation, the second term can be reformulated as:
\begin{equation} \label{eq:linear-expect-second-term}
\begin{aligned}
-2\eta\mathbb{E}_{(s,a)\sim\mu} \left(\sum_{l=1}^{L}\phi_{l}\phi^\top_{l}\right)&=-2\eta\sum_{l=1}^{L}\mathbb{E}_{(s,a)\sim\mu} \left(\phi_{l}\phi^\top_{l}\right)\\
&=-2\eta L \mathbb{E}_{(s,a)\sim\mu} \left(\phi(s,a)\phi(s,a)^\top\right)\\
&\preceq -\frac{2\eta L}{\kappa} \identity
\end{aligned}
\end{equation}


Next, we consider the third big expectation term. Specifically, for $1 \le l_1,\ldots, l_k \le L$ (and $2\le k\le 2L$),  consider one high-order term $\phi_{l_1}\phi^\top_{l_1}\ldots\phi_{l_k}\phi^\top_{l_k}$ in Equation~\eqref{eq:gamma-gamma}.  By Remark~\ref{rem:cauchy}, we have:
\begin{align}\label{eq:neighbor-inner-product}
|\phi^\top_{l_{j}}\phi_{l_{j+1}}|&=|\langle\phi_{l_j}, \phi_{l_{j+1}}\rangle|\le |\langle\phi_{l_j}, \phi_{l_{j+1}}\rangle|^2\le 1, \qquad \text{ for } 1\le j< k
\end{align}
Let $x\in\mathbb R^d$ be any $d$-dimensional non-zero vector. Based on the above analysis, we have:
\begin{align}
|x^\top\phi_{l_1}\phi^\top_{l_1}\ldots\phi_{l_k}\phi^\top_{l_k}x|&\le |x^\top \phi_{l_1} \phi^\top_{l_k} x|  &\text{by Equation~\eqref{eq:neighbor-inner-product}}\nonumber\\
 & \le \frac{1}{2}\left(\left(x^\top \phi_{l_1}\right)^2+ \left(\phi^\top_{l_k} x\right)^2\right)   &\text{AM-GM inequality in Lemma~\ref{lem:am-gm}}\nonumber\\
&= \frac{1}{2}\left(x^\top \phi_{l_1}\phi^\top_{l_1}x+x^\top\phi_{l_k}\phi^\top_{l_k}x \right) \nonumber\\
&= \frac{1}{2}x^\top\left( \phi_{l_1}\phi^\top_{l_1}+\phi_{l_k}\phi^\top_{l_k} \right)x
\end{align}
%  In terms of matrix positive semi-definitive (in Definition~\ref{def:psd}), we can conclude that:
% \begin{equation}  \label{eq:psd-head-tail}
%    -\frac{1}{2}\left( \phi_{l_1}\phi^\top_{l_1}+ \phi_{l_k}\phi^\top_{l_k} \right) \preceq \phi_{l_1}\phi^\top_{l_1}\ldots\phi_{l_k}\phi^\top_{l_k} \preceq \frac{1}{2}\left( \phi_{l_1}\phi^\top_{l_1}+ \phi_{l_k}\phi^\top_{l_k} \right) 
% \end{equation}
The above result implies only the first term indexed by $l_1$ and the last term indexed by $l_k$ determine the high order term $\phi_{l_1}\phi^\top_{l_1}\ldots\phi_{l_k}\phi^\top_{l_k}$. 




\begin{figure}[!t]
    \centering
    \includegraphics[width=0.85\linewidth]{fig/combinations-crop.pdf}
    \caption{Visualized case analysis for the possible combinations of picking entries from the arrays. [TODO:] explains this very clearly. a bunch of very complicated things. how and why the core part is }
    \label{fig:combination}
\end{figure}
 We then take into account the weighted summation $\sum_{k=2}^{2L}(-\eta)^k\sum_{l_1,\ldots,l_k}$ in Equation~\eqref{eq:gamma-gamma} thus obtain:
 \begin{equation}
\begin{aligned}\label{eq:comb}
\sum_{k=2}^{2L}(-\eta)^k&\sum_{l_1,\ldots,l_k}\frac{1}{2}( \phi_{l_1}\phi^\top_{l_1}+ \phi_{l_k}\phi^\top_{l_k} ) = \underbrace{\sum_{k=2}^{2L}(-\eta)^k\sum_{l=1}^L\left({L+l-2\choose k-1} +{L-l\choose k-1}+{2l-2\choose k-2}\right)}_{\text{sum over combinatorially many terms}}\phi_{l}\phi^\top_{l}
\end{aligned}     
 \end{equation}

As shown in Figure~\ref{fig:combination},  the element $\phi_{l}\phi^\top_{l}$  comes from the following cases:
\begin{enumerate}[label=(\alph*)]
    \item $(l_1=l\wedge l_k\neq l)$. This includes two subcases:
    \begin{enumerate}[label=(\arabic*)]
        \item $l_1$ could pick the left $l$  while the rest $k-1$ elements (\textit{i.e.,} $l_2,\ldots,l_k$) are picked from elements with  size $L+l-2$.
        \item $l_1$ picks the right $l$, and the rest  $k-1$ elements are picked from the subarray of  size $L-l$.
    \end{enumerate}
    \item $ (l_1\neq l\wedge l_k= l)$. This is symmetric to the above case, which also includes two subcases: 
    \begin{enumerate}[label=(\arabic*)]
        \item $l_k$ could pick the right $l$  while the rest $k-1$ elements (\textit{i.e.,} $l_1,\ldots,l_{k-1}$) are picked from elements with  size $L+l-2$. 
    \item $l_k$ picks the left $l$, and the rest  $k-1$ elements are picked from the subarray of  size $L-l$.
    \end{enumerate}
    \item  $(l_1=l \wedge l_k= l)$ and the rest $k-2$ elements are picked from subarray with size $2l-2$, when $2l\ge k$.  This case counts twice times for the $l$-th element. 
\end{enumerate}Note that the above .case (a) and (b) give the same result. Therefore, the $\frac{1}{2}$ coefficient are canceled in Equation~\eqref{eq:comb}.





% 

Based on the result in Equation~\eqref{eq:comb}, we have
\begin{align} \label{eq:upper-bound-third-term}
&\mathbb{E}_{(s,a)\sim\mu} \left(\sum_{k=2}^{2L}(-\eta)^k\sum_{l_1,\ldots,l_k}\frac{1}{2}( \phi_{l_1}\phi^\top_{l_1}+ \phi_{l_k}\phi^\top_{l_k}  ) \right)  \\
&\preceq \left( (1-\eta)^{2L}-\eta^2(1-\eta)^{2L-3}-\eta (1-\eta)^{L-1}  -1+\eta(2L+2)\right)\mathbb{E}_{(s,a)\sim\mu} \left(\phi(s,a)\phi(s,a
)^\top\right)  &\text{Lemma~\ref{lem:combi-weighted}}  \nonumber\\
&\preceq \frac{ (1-\eta)^{2L}-\eta^2(1-\eta)^{2L-3}-\eta (1-\eta)^{L-1}  -1+\eta(2L+2)}{\kappa}\identity &\text{Assumption~\ref{asump:phi-kappa}} \nonumber
\end{align}
Combining the results in Equation~\eqref{eq:linear-expect-second-term} and~\eqref{eq:upper-bound-third-term}, we finally have:
\begin{align*}
\mathbb{E}_{(s,a)\sim\mu}  \left(\Gamma_{L}^\top \Gamma_{L}\right) &\preceq \identity-\frac{2\eta L}{\kappa} \identity + \frac{ (1-\eta)^{2L}-\eta^2(1-\eta)^{2L-3}-\eta (1-\eta)^{L-1}  -1+\eta(2L+2) }{\kappa}\identity \\
&\preceq \left(1-\frac{\eta^2(1-\eta)^{2L-3}-(1-\eta)^{2L}+\eta (1-\eta)^{L-1}  +1-2\eta}{\kappa}\right)\identity
\end{align*}
The proof is thus finished.
